Understanding Persistent-Memory Related Issues in the Linux Kernel

Persistent memory (PM) technologies have inspired a wide range of PM-based system optimizations. However, building correct PM-based systems is difficult due to the unique characteristics of PM hardware. To better understand the challenges as well as the opportunities to address them, this paper presents a comprehensive study of PM-related issues in the Linux kernel. By analyzing 1,553 PM-related kernel patches in-depth and conducting experiments on reproducibility and tool extension, we derive multiple insights in terms of PM patch categories, PM bug patterns, consequences, fix strategies, triggering conditions, and remedy solutions. We hope our results could contribute to the development of robust PM-based storage systems

==> result.tex <==
%\vspace{-0.15in}
\subsection{Case Study I:~\texttt{e2fsck}}
\label{sec:e2fsck}



In this subsection, we apply the testing method to  study \texttt{e2fsck}.
As discussed in \S\ref{sec:background-undo},  \texttt{e2fsck} has recently added 
the  undo logging support. 
 For clarity, we name the original version without undo logging as  \texttt{e2fsck},
 and the version with undo logging as  \texttt{e2fsck-undo}.
%with and without the {undo} logging, respectively.
%Surprisingly, we observe similar unrecoverable corruptions in both cases.
%In other words, the current {undo} logging {cannot} prevent further damages caused
%by an interrupted check. Due to space limit, 
%we only present the results~\textit{with undo logging} in this section\footnote{
%The results of~\texttt{e2fsck} without undo logging can be found in our preliminary report~\cite{our_hotStorage13}.
%}.
%\fixme{update all numbers with undo logging}

We use  175 Ext4 test images from  \texttt{e2fsprogs}  v1.43.1~\cite{e2fsprogs} as inputs to trigger the checker. % \fixme{175 Ext2/3/4?}. %~\texttt{e2fsck}.
The sizes of these images range from 8MB to 128MB, and 
the file system block size is 1KB. %on all these images is 1KB. 
To emulate faults on storage systems with different atomic units, 
we inject faults
at two granularities:  512B and 4KB.  
In other words, we interrupt~\texttt{e2fsck} after every 512B or 4KB  of an I/O transfer command. 
Since the file system block is 1KB, we do not break file system blocks when injecting faults at the 4KB granularity. 

First, we study \texttt{e2fsck}  using the method in Figure~\ref{fig:workflow}a.
As described in \S\ref{sec:workflow}, for each fault injected (i.e., each interruption) we run \texttt{e2fsck} again and generate one repaired image.
From one test image we usually generate multiple repaired images because the repairing procedure usually requires updating 
multiple file system blocks.
For example, to fix the test image ``\texttt{f\_noroot}'' (image with no root directory) from \texttt{e2fsprogs},  \texttt{e2fsck} needs to update four 1KB blocks, which generates eight interrupted images (and consequently repaired images) when faults are injected after every 512B. 
%Among these 8 images, 4 images have reported "file content corruption" and other 4 have reported "misplacement of files".  
Table~\ref{tab:num_images} summarizes the total number of repaired images generated 
from the 175 test images at the two granularities.
%We can see that with the finer grain of fault injection (i.e., 512B), more repaired images are generated because the repairing procedure is 
We can see that  the 512B case leads to more repaired images (i.e., 25,062) because the repairing procedure is 
 interrupted more frequently. 


\begin{table}[tb]
\begin{center}
\begin{tabular}{c|c|c}
\hline
{\# of Ext4} & {Fault injection} & {Total \# of} \\
{test images} & {granularity}  & {repaired images} \\
\hline
\hline
175 & 512 B & 25,062  \\
175 & 4 KB & 3,195 \\
\hline
\end{tabular}
\end{center}
\vspace{-0.2in}
\caption{
{\bf Total number of repaired images.} 
{\it This table shows the number of repaired images generated from 175 Ext4 test images at two fault injection granularities.}
}
\label{tab:num_images}
\end{table}


\begin{table}[tb]
\begin{center}
\begin{tabular}{c|c|c}
\hline
{Fault injection} & \multicolumn{2}{c}{{\# of images reporting corruptions}} \\
\cline{2-3}
{granularity} & {test images}  & {repaired images} \\
\hline
\hline
512 B & 34 & 240  \\
4 KB & 17 & 37 \\
\hline
\end{tabular}
\end{center}
\vspace{-0.2in}
\caption{
%{\bf Number of Ext4 images reporting corruptions under two fault injection granularities.}
{\bf Number of images reporting corruptions. }
 {\it This table shows the number of Ext4 test images and repaired images reporting 
 corruptions at two fault injection granularities.}
%\fixme{add  undo logging results for the 17 or 34 images}
}
\label{tab:num_corruptions}
\end{table}

\begin{table}[t]
\begin{center}
\begin{tabular}{c|c|c}
\hline
{Corruption Type} & 512 B & 4 KB \\
\hline
\hline
{cannot mount} & 41 & 3 \\
{file content corruption} & 107 & 10 \\
{misplacement of files} & 82 & 23 \\
others & 10 & 1\\
\hline
Total & 240 & 37\\
\hline
\end{tabular}
\end{center}
\vspace{-0.2in}
\caption{
%\small{
%Number of  repaired images reporting each type of corruptions under two fault injection granularities.
{\bf Classification of corruptions.}
{\it This table shows the number of  repaired images reporting each type of corruptions at two fault injection granularities.}
}
\label{tab:normalresult}
\end{table}


By comparing with the reference image (Figure~\ref{fig:workflow}a), we can verify if a repaired image
contains unrecoverable corruptions or not. If at least one repaired image contains such corruption, we mark the corresponding test image
as reporting corruption, too. 
Table~\ref{tab:num_corruptions}  shows the numbers of test images and repaired images reporting  corruptions.
We can see that at the 512B granularity, more images have corruptions (e.g., 34  $>$ 17). This is because the updates are broken into smaller pieces,
and thus it is more challenging to maintain consistency when interrupted.


To further understand the severeness of the corruptions, 
we examine the symptoms  in  details and classify them into four types, including:
(1) \textit{cannot mount}; % file systems;
(2) \textit{file content corruption}; 
(3) \textit{misplacement of files} (e.g., a file is either in the``lost+found'' folder or completely missing)
(4) \textit{others} (e.g.,  showing ``???'' after an {\tt ls} command).  
Table~\ref{tab:normalresult} shows the number of  repaired images reporting each type of corruptions.
We can see that \textit{file content corruption} and \textit{misplacement of files}
are most common. Also, even at a fault injection granularity bigger than the file system block (i.e., 4KB $>$ 1KB), we still observe
three cases where the whole file system volume becomes not mountable  (i.e., ``cannot mount''). %becomes {unmountable}.
%Note that all these corruptions were observed 
%after running the checker again without interruption, 
%which means they cannot be recovered by the existing checker. 



\begin{table}[tb]
\begin{center}
\begin{tabular}{c|c|c}
\hline
{Fault injection} & \multicolumn{2}{c}{{\# of images reporting corruptions}} \\
\cline{2-3}
{granularity} & { e2fsck}  & { e2fsck-undo} \\
\hline
\hline
512 B & 34 & 34  \\
4 KB & 17 & 15 \\
\hline
\end{tabular}
\end{center}
\vspace{-0.2in}
\caption{
{\bf Comparison of e2fsck and e2fsck-undo.}
%{\bf Number of images reporting corruptions when testing e2fsck-undo. }
 {\it This table compares the number of test images reporting 
 corruptions under {e2fsck} and {e2fsck-undo}.}
 % two fault injection granularities when undo logging is enabled.}
%\fixme{add results}
}
\label{tab:num_corruptions-logging}
\end{table}

Next, to see if the undo logging can avoid the corruptions, % caused by \texttt{e2fsck}, 
we use the method in Figure~\ref{fig:workflow}b to study \texttt{e2fsck-undo}.
We focus on the test images  which report
corruptions when testing \texttt{e2fsck} (i.e., the 34 and 17 test images in Table~\ref{tab:num_corruptions}).% at the 4 KB fault injection granularity.

Table~\ref{tab:num_corruptions-logging} compares the number of test images reporting 
 corruptions under \texttt{e2fsck} and \texttt{e2fsck-undo}. 
 Surprisingly, we observe a similar amount of corruptions.
 %at both granularities \fixme{wait for result}. 
 For example, all 34 images which report corruptions when testing \texttt{e2fsck} at the 512B granularity 
 still report corruptions under \texttt{e2fsck-undo}.
 We defer the analysis of the root cause to \S\ref{sec:why}.



==> sys_bugtools.tex <==
\section{PM Bug Detection Tools}
\label{sec:bug_tools}

